Data-centric Prediction Explanation via Kernelized Stein Discrepancy

Existing example-based prediction explanation methods often bridge test and training data points through the model's parameters or latent representations. While these methods offer clues to the causes of model predictions, they often exhibit innate shortcomings, such as incurring significant computational overhead or producing coarse-grained explanations. This paper presents a Highly-precise and Data-centric Explan}ation (HD-Explain) prediction explanation method that exploits properties of Kernelized Stein Discrepancy (KSD). Specifically, the KSD uniquely defines a parameterized kernel function for a trained model that encodes model-dependent data correlation. By leveraging the kernel function, one can identify training samples that provide the best predictive support to a test point efficiently. We conducted thorough analyses and experiments across multiple classification domains, where we show that HD-Explain outperforms existing methods from various aspects, including 1) preciseness (fine-grained explanation), 2) consistency, and 3) computation efficiency, leading to a surprisingly simple, effective, and robust prediction explanation solution.

==> reviews.tex <==

We are immensely grateful for the time and effort invested by all the reviewers. It brings us great pleasure to see that all reviewers unanimously acknowledged the novelty of our research and commended the direction of our work.

U5g9 highlighted that the correlation properties of KSD in our novel idea shed new light on prediction explanation. E1tX praised the simplicity and ease of implementation of our method, in addition to its performance compared to previous works. R8od indicated that our work exhibited substantial promise. Finally, reviewers gEo5 and r8od appreciated the experimental study conducted on different datasets. 

We noted some commonalities in the questions asked, so we addressed these topics together.

The experimental evaluation on the SOTA; We observed that reviewers were concerned about the lack of more experimental evaluations and comparisons with SOTA baselines. Due the limited time in the rebuttal period, we are planning to conduct the experimental comparison during the revision time. 

Regarding the clarity of our work and the , (pairing the comments of reviewers U5g9, gEo5, and r8od ) specifically regarding the motivation of Kernelized Stein Discrepancy (KSD) and the formulation of KSD conditioned on the model, we refer back to our paper. As per the noted comments from the reviewers, Stein’s identity provides a mechanism to measure the gap between two distributions by assuming that the variable $x$ is sampled from a different distribution $q \neq p$ such that 
\[\sqrt{\mathbb{S}(q,p)} = \max_{\phi\in\mathcal{F}}\mathbb{E}_{x\sim q}[\mathcal{A}_p\phi(x)],\]
where the expression takes the most discriminant $\phi$ that maximizes the violation of Stein's identity to quantify the distribution discrepancy. Intuitively, by using integration by part rules, we can reveal the original assumption from the derived expression such that
\[    \int_x\phi(x)\nabla_{x}\log p(x) + \nabla_x \phi(x) dx = p(x)\phi(x)\Bigr|^{+\infty}_{-\infty} \]

The Stein Discrepancy quantifies the disparity between two distributions $q$ and $p$ by substituting the expectation of the distribution $p$ term in Stein's Identity expression with that of distribution $q$. This substitution unveils the discrepancy between the two distributions by projecting their score functions (gradients) using the function $\phi(x)$:
\[\max_{\phi\in \mathcal{F}}\mathbb{E}_{x\sim {\color{orange!80}q}} [\mathcal{A}_p\phi(x)] = \max_{\phi\in \mathcal{F}} \mathbb{E}_{x\sim {\color{orange!80}q}} [\mathcal{A}_p\phi(x)] - \underbrace{\mathbb{E}_{x\sim {\color{orange!80}q}} [\mathcal{A}_{\color{orange!80}q}\phi(x)]}_{=0} = \max_{\phi\in \mathcal{F}} \mathbb{E}_{x\sim {\color{orange!80}q}} [\underbrace{\phi(x)}_{\text{projection coefficients}}\underbrace{(\nabla_x\log p(x)-\nabla_x\log {\color{orange!80}q}(x))}_{\text{score function difference}}]
\]

Recall that the Kernelized Stein Discrepancy (KSD), denoted as $\mathbb{S}(P_D, P_\theta)$, characterizes the correlation between pairs of training samples through a model $\theta$-dependent kernel function with a closed-form decomposition:

\begin{equation}
\begin{aligned}
    &\kappa_\theta ((\mathbf{x}_a, y_a), (\mathbf{x}_b, y_b)) =  \mathcal{A}_\theta^a\mathcal{A}_\theta^{b} k(a, b)\\
    &= \nabla_a\nabla_b k(a,b) + k(a,b) \nabla_a \log P_\theta(a) \nabla_b \log P_\theta(b)\\
    &+\nabla_a k(a,b)\nabla_b\log P_\theta(b) + \nabla_b k(a,b) \nabla_a \log P_\theta(a),
\end{aligned}
\label{eq:ksd_kernel_function}
\end{equation}
 

Thus, in order to employ KSD for explaining predictions, our initial step involves uncovering the derivative of the trained model concerning an entire data point, and setting $P_\theta(\mathbf{x}) \equiv P_D(\mathbf{x})$ as a uniform distribution. With this setting, the score function could be derived as a concatenation of the gradient of the model to its input and its probabilistic prediction. Finally, we can estimate the correlation of any pairs of training data points conditioned on the trained machine learning model.

Questions and requests - R1:

Why is our algorithm considered to be a Highly Precise explanation method? Why is using KSD highly precise? (Other algorithms also provide the per-instance explanation) 

We introduce our method as Highly Precise Explanation due to sound statistical background of the KSD and findings illustrated in our Qualitative Evaluation (Figures 6 and 7)., for the different target data points the majority of baseline algorithms are showing the same explanation to those different instances showing. Even per-instance explainer methods experience significant collapse in their explanations across different instances. However, our method offers distinct explanations, greater diversity, and broader coverage across all test cases in the experiments.


What is the advantage of data correlation explanation over the influence-based method? As highlighted in our motivation section and further emphasized by Reviewer r8od, influence-based explainers tend to be computationally demanding. This computational expense can arise due to the need to assess the impact of individual data points on the model's predictions, which can become particularly burdensome in scenarios involving large datasets or complex models. Additionally, influence-based methods often require extensive computational resources to calculate the influence of each data point accurately. Conversely, data correlation explanations offer a potentially more efficient alternative by focusing on understanding how different features correlate with the model's predictions. This approach can provide valuable insights into the model's decision-making process without the computational overhead associated with influence-based methods. Furthermore, data correlation explanations can offer a more intuitive understanding of the model's behavior by highlighting the relationships between features and predictions, making them particularly useful for interpretability and debugging purposes.
What is the motivation for the employment of KSD?
Our motivation for the employment of KSD, as mentioned in our paper is that the concept of Kernelized Stein Discrepancy originates from a sound statical theorem known as Stein's Identity. This theorem provides a means to quantify the disparity between two distributions even when the normalizing factor of the target distribution is unavailable. Through the innovation of KSD, the Stein operator augmented kernel uniquely defines pairwise data correlation within the context of a trained model. Its expectation on the training dataset minimizes the KSD, serving as a discrete approximation when compared to datasets sampled from different distributions. By leveraging this property, we can achieve two objectives: 1) pinpoint a subset of training data points that offer the best predictive support for a given test point and 2) detect potential distribution mismatches among the training data points.

How does our model retain the influence chain between the training and test? Show the formula? 
To understand the chain of influence between the test data and training samples we should take a look at the definition of KSD. As we mentioned in the paper KSD is a parameterized kernel that measures the correlation between each test datapoint and train point. Intuitively, the connection shows that there is a tie between a model and its training data points, encoded in the form of a stein kernel function $k_\theta(\cdot, \cdot)$ defined on each pair of data points. As the kernel function is conditioned on model $f_\theta$, we note it is an encoding of data correlation under the context of a trained model, which paves the foundation of the example-based prediction explanation as shown next.

Is there an intuitive meaning for the Stein operator? You cite Liu & Wang which show that minimizing KL divergence is equivalent to the direction the stein discrepancy, so what additional viewpoint do we gain by considering Stein discrepancy?

Requests:

Label the KSD values on the gradient color map
Increase the size of the black cross in the figure
Discuss the KSD values of several datapoints in the Figure, why some of them have high KSD value?
More discussion about the experimental results, Does our algorithm perform better in all cases? If not, discuss when it fails or where others excel? 


Repeat the experiments to avoid cherry picking data
For the explanation procedure, draw a sample from test set and explain it with the training samples?
The execution time of HD-Explain is mediocre and it doesn’t beat all other baselines

-------------------------------------------------------------------------------------------------------------------------------

Questions and requests - R2:

Requests:
Compare your algorithm with SOAT such as 
https://arxiv.org/abs/2303.14186
https://arxiv.org/abs/2202.00622
https://arxiv.org/abs/2308.03296


-------------------------------------------------------------------------------------------------------------------------------

Questions and requests - R3:

Requests:
Review the existing works about the importance of example-based prediction explanation, especially since most models consider training data is not available.
We are planning to discuss the importance of example based prediction more comprehensively in our revision. Here is a brief draft of it:
 Explaining the predictions made by complex machine learning models helps users
to understand and accept the predicted outputs with confidence. One promising way
is to use a similarity-based explanation that provides similar instances as evidence
to support model predictions. Showing an example of instances from a training dataset would be a beneficial data-centric explanation of the model inferences (Molnar, 2022). In particular, an example similar to the inferred target data would be a valuable reference to verify whether the model is trained on a dataset sufficiently close to the target data (Hanawa et al., 2021). If the most similar example is too far away from the target, we can interpret that it is invalid to apply the model to the target data, and the inference result is suspicious.

Molnar, Christoph. Interpretable machine learning. Lulu. com, 2020.

Hanawa, Kazuaki, et al. "Evaluation of similarity-based explanations." arXiv preprint arXiv:2006.04528 (2020).


Clearly state the advantage of KSD compared to other distance measure
The difference between KSD and others: 1. KSD-defined pair-wise distance is a parameterized distance metric that is conditioned on the original model's parameters. It naturally included the similarity of features, the similarity of score functions, and even the similarity of data labels, without introducing manually defined hyper-parameters. Many classic distance metrics do not cover all of the three similarity factors mentioned above.


The predicted label information is utilized to compute the KSD, use the whole softmax probability distribution
Clear the “WHole model explanation” in Table 1
The whole model explainer states that all parameters of the model participate in the generated explanation.
State why the theoretical checkmark is marked for the proposed method in Table 1.
Conducting an ablation study to adjust the noise variance when adding noise to the training samples would be advantageous
Explain why HD-Explain* underperforms on CIFAR10 but excels on OCH

-------------------------------------------------------------------------------------------------------------------------------

Questions and requests - R4:

How are the computational gain measured?  From a look at the code it seems the wall time is total, while one would focus on constructing gradients (or reducing their dimensionality with FAISS) as the search can be amortized [GS]; an observation from [GS] that undermines efficiency claims is that you can store the gradient in compressed form using FAISS, while in the KDS-method proposed by the authors the data to store will grow like the input; in particular for NLP sequences on realistic tasks this would grow much more than in the cases considered in the paper. Further reason to worry: your method requires a full backward pass while TraceIn on the last layer costs more or less like a forward pass, so it would important to have the breakdown of how to measure computational gains.


As introduced HD-Explain* in the paper, it represents a straightforward modification of HD-Explain, involving the utilization of data representations (specifically, the output of the last non-predictive layer of the neural classifier) rather than raw features. Specifically, we consider a neural network model $f_\theta$ that can be decomposed into two components: $f_{\theta_2} \cdot f_{\theta_1}$, where $f_{\theta_1}$ serves as a representation encoder and $f_{\theta_2}$ functions as a linear model for prediction. Within this decomposition framework, we define the KSD kernel function for HD-Explain* as follows:

\[
\begin{aligned}
    &\kappa_\theta ((f_{\theta_1}(\mathbf{x}_a), y_a), (f_{\theta_1}(\mathbf{x}_b), y_b)) =  \mathcal{A}_{\theta_2}^a\mathcal{A}_{\theta_2}^{b} k(a, b)\\
    &= \nabla_a\nabla_b k(a,b) + k(a,b) \nabla_a \log P_{\theta_2}(a) \nabla_b \log P_{\theta_2}(b)+\nabla_a k(a,b)\nabla_b\log P_{\theta_2}(b) + \nabla_b k(a,b) \nabla_a \log P_{\theta_2}(a),
\end{aligned}
\]


where $a = (f_{\theta_1}(\mathbf{x}a), y_a)$ and $b = (f{\theta_1}(\mathbf{x}_b), y_b)$ for brevity. This framework effectively reduces the prediction explanation process to the last layer of the neural network, akin to RPS.

Requests:
Normalizing the calc\_influence\_function In “tracin.py” uses the pure product of gradients instead of normalizing them
ksd.py: in practice you construct it with [$nabla_x log P(y|x), P(y|x)$], but in the paper you talk about taking a $\nabla_y$, which is unclear also because y is discrete
Check the construction of KSD in code w.r.t the formula presented in the paper
What does the similarity score $KSD(x_i, x_j)$ between two datapoint points out? 
To understand the similarity score between two datapoints we should decompose the function and examine each part. 
In HD-Explain, the key metric on measuring the predictive supports of a test point $\mathbf{x}_t$ given a training data $(\mathbf{x}_i, \mathbf{y}_i)$ is the KSD defined kernel $\kappa_\theta([\mathbf{x}_t||\hat{\mathbf{y}}_t], [\mathbf{x}_i||\mathbf{y}_i])$, where $\hat{\mathbf{y}}_t$ denotes the predicted class label by model $f_\theta$ in one-hot encoding. By definition, the kernel $\kappa_\theta ((\mathbf{x}_a, y_a), (\mathbf{x}_b, y_b)) = k_\theta(a,b)$ between two data points can be decomposed into four terms
\[
     \underbrace{\text{trace}(\nabla_a\nabla_b k(a,b))}_{\text{\ding{172}}} + \underbrace{k(a,b) \nabla_a \log P_\theta(a)^\top \nabla_b \log P_\theta(b)}_{\text{\ding{173}}} +\underbrace{\nabla_a k(a,b)^\top\nabla_b\log P_\theta(b)}_{\text{\ding{174}}} + \underbrace{\nabla_b k(a,b)^\top \nabla_a \log P_\theta(a)}_{\text{\ding{175}}}.
\]

We examine the effect of each term as follows:
\begin{itemize}
    \item \ding{172}: We note that the first term is often a similarity bias of raw data points given a specified kernel function. In particular, for the RBF kernel $ k(a,b) = \exp(-\gamma||a - b||^2)$, the first term is simply $\sum_{i}^{d+l} 2\gamma k(a, b)$, where $d+l$ refers to the sum of input and output (in one-hot) dimensions of a data point. Intuitively, the term shows how similar the two data points are given the RBF kernel. For linear kernel $k(a,b) = a^\top b$, on another hand, the first term is simply $d+l$ as a constant bias term, which does not deliver any similarity information between the two data points. 
    \item \ding{173}: The second term reflects the similarity between two data points in the context of the trained model. In particular, considering the sub-term $\nabla_a \log P_\theta(a)^\top \nabla_b \log P_\theta(b)$, based on our derivation in Equation~\ref{eq:score_function} (in the main paper), we note it is equivalent to
    \[[\nabla_{\mathbf{x}_a}\log f_\theta(\mathbf{x}_a)_{y_a} || f_\theta(\mathbf{x}_a)]^\top [\nabla_{\mathbf{x}_b}\log f_\theta(\mathbf{x}_b)_{y_b} || f_\theta(\mathbf{x}_b)] = \underbrace{\nabla_{\mathbf{x}_a}\log f_\theta(\mathbf{x}_a)_{y_a}^\top \nabla_{\mathbf{x}_b}\log f_\theta(\mathbf{x}_b)_{y_b}}_{\text{similarity of scores  (input gradients)}} +  \underbrace{f_\theta(\mathbf{x}_a)^\top f_\theta(\mathbf{x}_b)}_{\text{similarity of predictions}},\]where both terms could be viewed as similarity between data points in the context of trained model.
    \item \ding{174}-\ding{175}: Both of the last two terms examine the alignment between the score of one data point and the kernel derivative of another data point. We conjecture that this alignment reflects how a test prediction would change if there is a training data point present closer to it than before.  
\end{itemize}


-------------------------------------------------------------------------------------------------------------------------------

Questions and requests - R5:

Although finding the most correlated training examples makes sense, how the idea of KSD helps in explaining the model?
KSD is a great summary of the machine learning model it is a prototype and a great summary of the machine learning model (from the existing literature). The prototyping approach means that with a small number datapoints, we can identify the most influential datapoints for the model. KSD is a prototyping solution not just an explanation. In summary, the Kernelized Stein Discrepancy serves as a measure of how well each data point represents the overall distribution of the dataset. By selecting points with high KSD values, we select prototypes that capture the essential characteristics of the data distribution, making them suitable for downstream tasks. Therefore, KSD can indeed be considered a prototype data selection method.

Liu, Qiang, and Jason D. Lee. "Stein Variational Gradient Descent: A General Purpose Bayesian Inference Algorithm." Advances in Neural Information Processing Systems. 2016. (Link)

Gorham, Jackson, and Lester Mackey. "Measuring sample quality with Stein’s method." In Advances in Neural Information Processing Systems, pp. 226-234. 2015. (Link)

Why instead of KSD, we do not use the linear kernel on the learned embedding as the covariance measure?
Linear kernel introduces some artifacts outside of the original model, the KSD is the natural measure that only incorporates the elements of the machine learning model by itself. The KSD is defined by the machine learning model by itself, all parameters are obtained from the model. The main problem of linear kernels is introducing additional parameters, and if we discuss the linear kernel, we should also consider non linear kernels. Additional drawback of linear kernel is taking the only learned embedding and it ignores the rest of the model in obtaining the correlations. You only looking ar the similarity of train and test points from based on the embedding layer, using the linear kernel ignores the last prediction layer, also it only partially uses the information within the model
Requests:

Considering the marginal distribution $P_\theta$ as a uniform distribution is not enough. To ensure that considering the original distribution as uniform doesn’t affect which training examples are selected, We treat each datapoint as IID and naturally, this is considered to be a uniform distribution.
In this paper “[1] Grathwohl, W., Wang, K. C., Jacobsen, J. H., Duvenaud, D., Norouzi, M., & Swersky, K. (2019). Your classifier is secretly an energy based model and you should treat it like one. arXiv preprint arXiv:1912.03263.” the logsumexp of any classifier can be interpreted as an unnormalized marginal log density so no changes to the model is necessary to estimate $\nabla_x \log p_\theta(x)$
More discussion on why the examples returned by HD-Explain in Figures 3 and 4 are visually better than the those from the alternative methods. 
By taking a close look at the extracted explanation from Figure 3 on Highly confident correct prediction, the obtained correlated samples are more similar in terms of Frog’s posture, color palette of picture, the position of frog in the picture. However, when we look into other methods, the top influential training data do not display a similar quality.

